Krutrim LLM: A Novel Tokenization Strategy for Multilingual Indic Languages with Petabyte-Scale Data Processing

We present a novel approach to data preparation for developing multilingual Indic large language model. Our meticulous data acquisition spans open-source and proprietary sources, including Common Crawl, Indic books, news articles, and Wikipedia, ensuring a diverse and rich linguistic representation. For each Indic language, we design a custom preprocessing pipeline to effectively eliminate redundant and low-quality text content. Additionally, we perform deduplication on Common Crawl data to address the redundancy present in 70% of the crawled web pages. This study focuses on developing high-quality data, optimizing tokenization for our multilingual dataset for Indic large language models with 3B and 7B parameters, engineered for superior performance in Indic languages. We introduce a novel multilingual tokenizer training strategy, demonstrating our custom-trained Indic tokenizer outperforms the state-of-the-art OpenAI Tiktoken tokenizer, achieving a superior token-to-word ratio for Indic languages.

==> files/experiments_and_results.tex <==

\section{Experiments and Results}

\subsection{Pre-training Results} 
%  Pre-training Results with d/f Tokenizers
%  Pre-training Results with d/f dataset (unfiltered, filtered, deduped)
%  Pre-training Results comparision with SOTA and famous benchmarks

We have trained language models with 3 billion and 7 billion parameters, utilizing tokenizers with varying vocabulary sizes. The datasets employed in training varied in terms of the extent of cleaning and filtering, as well as in their compositional diversity. Pretraining was conducted on a setup comprising 240 H100 GPUs. Our models leverage the MPT architecture, with a maximum sequence length of 2048, 32 layers, embedding size of 2560, and 20 attention heads, each with a dimension of 128. Our model incorporates multi-head attention with rotary position embedding with a rotary dimension of \textcolor{red}{\textbf{ XXX }}. Our experiments involved the use of custom multilingual tokenizers with vocabulary sizes of 70,000, 80,000, and 100,000.




\begin{table}[h]
\centering
\captionsetup{justification=centering,}
\scriptsize
\begin{tabular}{
  |>{\centering\arraybackslash}p{1.7cm}|
   >{\centering\arraybackslash}p{1cm}|
   >{\centering\arraybackslash}p{1cm}|
   >{\centering\arraybackslash}p{1cm}|
   >{\centering\arraybackslash}p{1cm}|
   >{\centering\arraybackslash}p{1cm}|
   >{\centering\arraybackslash}p{1cm}|
}

\hline
\textbf{Dataset} & \textbf{Tokenizer} & \textbf{Model Size }& \textbf{ IndicGlue Score} \\
\hline
Basic filtered CC & 70K & 0 & 0 \\
Full filtered CC & 70K & 0 & 0 \\
Deduplicated CC & 70K & 0 & 0 \\
Basic filtered CC & 80K & 0 & 0 \\
Full filtered CC & 80K & 0 & 0 \\
Deduplicated CC & 80K & 0 & 0 \\
Basic filtered CC & 100K & 0 & 0 \\
Full filtered CC & 100K & 0 & 0 \\
Deduplicated CC & 100K & 0 & 0 \\\hline
\end{tabular}
\caption{Performance Metrics  with different Tokenizers and Common Crawl Dataset}
\label{tab:dataset experiments}
\end{table}

\textbf{Discussion for table \ref{tab:dataset experiments} . . . . . . . .}


\begin{table}[h]
\centering
\captionsetup{justification=centering,}
\scriptsize
\begin{tabular}{
  |>{\centering\arraybackslash}p{1.7cm}|
   >{\centering\arraybackslash}p{1cm}|
   >{\centering\arraybackslash}p{1cm}|
   >{\centering\arraybackslash}p{1cm}|
   >{\centering\arraybackslash}p{1cm}|
   >{\centering\arraybackslash}p{1cm}|
   >{\centering\arraybackslash}p{1cm}|
}

\hline
\textbf{Dataset Composition} & \textbf{Model Size }& \textbf{ IndicGlue Score} \\
\hline
CC(50\%), Newspaper(25\%), Books(25\%) & 3B & 0 \\
CC(50\%), Newspaper(25\%), Books(25\%) & 3B & 0 \\
CC(50\%), Newspaper(25\%), Books(25\%) & 3B & 0 \\\hline
\end{tabular}
\caption{Performance Metrics  with different data mixes}
\label{tab:dataset-mix experiments}
\end{table}

\textbf{Discussion for table \ref{tab:dataset-mix experiments}  . . . . . .}




==> files/tokenizer_old.tex <==
\section{Experiments and Results}
\subsection{Tokenizer}
A tokenizer is a piece of software used in computer science and natural language processing (NLP) that divides a text or character string into smaller parts called tokens. Tokens are generally words, sentences, or other significant items that serve as the fundamental building blocks of natural language processing. Tokenization is an essential step in many NLP jobs that enables computers to comprehend and interpret human language.
Basically toknizer comes in four varients, word Tokenization, sentence Tokenization, character tokenization, sub word tokenization.

SentencePiece\cite{kudo2018sentencepiece} differs from other subword segmentation tools by training subword models directly from raw sentences, enabling a fully end-to-end and language-independent system, without relying on pre-tokenized word sequences.





\subsection{Tokenizer details}
Numerous experiments were conducted prior to the introduction of Tokenizer-2, as detailed in Section 4.2.2. Further elaboration on these experiments is provided in the appendix. The experiments began by varying the size of the training corpus to 10k, 16k, 25k, 32k, and 64k for both 1B and 2B datasets, with a focus on examining the disparity in unique tokens. The findings revealed that there was no significant alteration in tokens.

Subsequently, separate tokenizer training sessions were initiated for Hindi and Telugu language data, employing training corpora sizes of 1B, 100M, 20M, and 10M. The analysis indicated a consistent absence of impact on common tokens, especially evident in the "Alphabet size" of Llama, between the 2B and 20M Hindi corpora and the 2B and 100M Telugu corpus. Exploration into character coverage values of 0.9995, 0.9998, and 1 revealed a lower count of missing base characters in each language under a character coverage of 0.9998.

Comparison of fundamental characters between Hindi and Marathi, as well as Assamese and Bengali, showcased considerable similarity. A detailed examination of shared tokens in the vocabularies of these languages demonstrated more than 5,000 shared tokens between Hindi and Marathi, and over 3,000 between Assamese and Bengali. A comprehensive account of this preliminary investigation is provided in the appendix.

Utilizing this insight, the establishment of three tokenizers ensued, each to be trained with 70k, 85k, and 100k tokens, with specific details outlined in Section 4.2.2.

% We ran numerous experiments before moving on to Tokenizer-2 in section 4.2.2; further information on these experiments can be found in the appendix section. When the size of the training corpus was increased to 10k, 16k, 25k, 32k, and 64k with 1B and 2B, the difference in unique tokens was examined. The result showed that tokens did not change significantly.We began training tokenizer of hindi and telugu languge data seperately with 1B, 100M, 20M, and 10M data. We discovered that there was no influence on common tokens with "Alphabet size" of Llama between 2B and 20M training corpus in hindi and 2B and 100M traing corpus of telugu language. While experimenting with character coverage 0.9995,0.9998 and 1, it was discovered that the number of missing base characters is lower in each language with character coverage of 0.9998.The fundamental characters for the Hindi and Marathi languages are nearly identical and checked number of tokens shared by the two languages' vocabularies which is true for the Assamese and Bengali languages. There are over 5,000 shared tokens between Hindi and Marathi, and 3,000 between Assamese and Bengali. All of this preliminary work is described in detail in the appendix section.With this information, we could set up three tokenizers to be trained with 70k, 85k, and 100k tokens. Specifics are covered in section 4.2.2.
\subsubsection{Tokenizer-1}\

\subsubsection{Tokenizer-2}\
\textbf{Data Sampling: } Data was sampled from four sources: Wikipedia, AI4Bharat, PDF, and Common Crawl. collected 5M, with the exception of "Hindi", "Marathi" and "English" from every source. We gathered 25 million data points for Hindi and 15 million for Marathi, and we only used Wikipedia for English data. We processed this data using fallbacks to remove most Chinese data and a few other emogis.


\textbf{Tokenizer settings :}


\\
\begin{table*}[h]
\centering
{%
\begin{tabular}{|>{\centering\arraybackslash}p{2cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|}
\hline
Tokenizer&  
en&
hi+mr&
te&
ta&
bn+as&
gu&
kn&
ml&
od&
pn
\\
\hline
70K&
16&
12&
5&
5&
7&
5&
5&
5&
5&
5
\\
\hline
85K&
24&
14&
6&
6&
7&
6&
6&
6&
5&
5
\\
\hline
100K&
32&
16&
7&
7&
8&
6&
6&
6&
6&
6
\\
\hline
\end{tabular}
}
\caption{Tokenizer -2 settings}

\end{table*}
% \FloatBarrier
\\

\\
\begin{table*}[h]
\centering
{%
\begin{tabular}{|>{\centering\arraybackslash}p{2cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|}
\hline

% |p{2cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|
Tokenizer&  
en&
hi+mr&
te&
ta&
bn+as&
gu&
kn&
ml&
od&
pn
\\
\hline
70K&
\textasciitilde15.4&
\textasciitilde14&
\textasciitilde5.4&
\textasciitilde4.7&
\textasciitilde6.6&
\textasciitilde4.7&
\textasciitilde4.4&
\textasciitilde5.2&
\textasciitilde5.3&
\textasciitilde6.3
\\
\hline
85K&
\textasciitilde23.2&
\textasciitilde16.3&
\textasciitilde7&
\textasciitilde6&
\textasciitilde6&
\textasciitilde6&
\textasciitilde6.1&
\textasciitilde5.5&
\textasciitilde6&
\textasciitilde5.2
\\
\hline
100K&
\textasciitilde31&
\textasciitilde16.6&
\textasciitilde7.5&
\textasciitilde7.1&
\textasciitilde8.5&
\textasciitilde6.2&
\textasciitilde6.3&
\textasciitilde6.4&
\textasciitilde6.5&
\textasciitilde5.7
\\
\hline
\end{tabular}
}
\caption{Tokenizer -2 vocabulary for each language}

\end{table*}
% \FloatBarrier
\\
\textbf{Approach: }
The data was cleaned by eliminating the unk tokens using trained tokenizers with vocabulary sizes of 70k, 85k, and 100k without fallback. Trained the final tokenizers of vocabulary size 70k,85k,100k on the cleaned data and obtained the good token to word ratio of each language.

\subsection{Tokenizer Evaluation Metrics}\


\textbf{Token to word ratio :} The token-to-word ratio refers to the relationship between the number of tokens and the number of words in a given text. The "tokens" can be words, subwords, or characters, depending on the tokenization strategy
A higher token-to-word ratio indicates that the text is tokenized into smaller units, which might be useful for tasks that require capturing fine-grained linguistic details. However, it also means that the text representation might be more detailed and the vocabulary larger.\

\textbf{Exact Score :}
It measures how well the tokenizer correctly identifies and segments the text into the expected units.Basically the ratio of the no of correct tokens to the total tokens.\

\textbf{Cosine Similarity :}
Calculate the cosine similarity between the embeddings of the original and tokenized sequences
Higher cosine similarity values indicate greater similarity in the vector representations, suggesting that the tokenizer has preserved the semantic meaning of the input. Averaging the cosine similarity across a set of words or sentences, to assess the overall performance of the tokenizer.\


\subsection{Tokenizer Results}

We conducted training using three tokenizer configurations: 70k, 85k, and 100k. The outcomes are presented in Table 5. Analysis reveals that augmenting the tokenizer vocabulary size from 70k to 85k and 100k results in reduced token-to-word ratios. Consequently, any tokenizer may be employed for the specific use case. Notably, the utilization of the 70k tokenizer yields lower inference times compared to the other configurations.


\begin{table*}[h]
\centering
{%
\begin{tabular}{|>{\centering\arraybackslash}p{2cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|>{\centering\arraybackslash}p{0.8cm}|}

\hline
Tokenizer&
en&
hi&
mr&
te&
ta&
as&
gu&
kn&
ml&
od&
pn
\\
\hline
T-1&
1.44&
3.64&
4.94&
5.97&
6.87&
4.52&
4.0&
5.7&
7.73&
4.67&
3.25
\\
\hline
T-2 (70k)& 
1.52&
1.38&
1.83&
2.58&
2.51&
2.06&
2.05&
2.51&
3.01&
1.94&
1.58
\\
\hline
T-2 (85k)& 
1.49&
1.36&
1.83&
2.45&
2.41&
2.03&
1.92&
2.32&
2.98&
1.89&
1.66
\\
\hline
T-2 (100k)& 
1.46&
1.35&
1.79&
2.39&
2.30&
2.00&
1.90&
2.29&
2.86&
1.85&
1.63
\\
\hline
\end{tabular}
}
\caption{Comparision of Tokenizer-1 and Tokenizer-2}

\end{table*}
\FloatBarrier




==> files/wiki.tex <==
\subsection{Indic-Wikipedia}
